Testing High-Energy Emission Models for Blazars with X-ray Polarimetry

Both leptonic and hadronic emission processes may contribute to blazar jet emission; which dominates in blazars's high energy emission component remains an open question. Some intermediate synchrotron peaked blazars transition from their low to high energy emission components in the X-ray band making them excellent laboratories to probe both components simultaneously, and good targets for the newly launched Imaging X-ray Polarimetry Explorer. We characterize the spectral energy distributions for three such blazars: CGRaBS~J0211+1051, TXS~0506+056, and S5~0716+714, predicting their X-ray polarization behavior by fitting a multizone polarized leptonic jet model. We find that a significant detection of electron synchrotron dominated polarization is possible with a 300~ks observation for S5~0716+714 and CGRaBS~J0211+1051 in their flaring states, while even 500~ks observations are unlikely to measure synchrotron self-Compton polarization. Importantly, non-leptonic emission processes like proton synchrotron are marginally detectable for our brightest ISP, S5~0716+714, during a flaring state. Improved {\it IXPE} data reduction methods or next generation telescopes like {\it eXTP} are needed to confidently measure SSC polarization.

==> ISP paper pre S5 (3)/referee_response.tex <==
\begin{document}
\textbf{Referee Response}

However, the model is not sufficiently described. It is hard to determine if the model assumptions can broadly reflect the true physical conditions in these blazars. Additionally, there is a previous work on TXS 0506+056 high-energy polarization, which appears to predict slightly different polarization degree. Therefore, I would recommend the authors to expand their description and discussion. It may be better to move the paper to ApJ.
 
1.	Page 1, since both electron synchrotron, proton synchrotron, and pair synchrotron are mentioned in the text, it would be good to explicitly distinguish them to avoid confusion. For instance, in line 57 "the synchrotron" probably means electron synchrotron, in line 58 "synchrotron" probably means electron synchrotron as well, but if the authors refer to the proton synchrotron, depending on the parameters, protons may not cool efficiently in the blazar zone. As long as the acceleration continues, protons can fill up most of the blazar zone easily.

Where appropriate throughout the text, reference to "synchrotron" emission has been disambiguated, making clear where we mean primary electron synchrotron, proton synchrotron, and secondary pair cascade synchrotron.

2.	Page1, line 61, "this means ...". This statement is generally true. However, PIC simulations suggest that the particles and magnetic field distributions are quite chaotic in the turbulent region. In that case, even though there are less cells with high-energy particles, the local PA is very disordered, so that the Stokes parameters can still be canceled easily.

Qualified the statement by noting that this also increases polarization variability, line 62.
As long as downstream of the acceleration region the magnetic fields are equally chaotic, averaging over fewer magnetic field zones always increases the expected (average) polarization. 
We discuss the case where magnetic fields are more or less chaotic close to the acceleration region (than downstream) in more detail in section 4, line 333. Here we mention that immediately downstream of a shock, magnetic fields are more likely to be perpendicular to the shock normal.

3.	Page 2, line 71, "proton-synchrotron". Most leptohadronic models of TXS 0506+056 use photomeson initiated hadronic cascading pair synchrotron to explain the neutrino event and fit SED, including Gao et al. Proton synchrotron is only discussed by very few works, and in those works, proton synchrotron generally dominates the high-energy spectral component. I assume the authors mean the subdominant pair synchrotron.

We have disambiguated "proton synchrotron", line 73; we indeed meant synchrotron from proton initiated cascades. See point 1.

4.	Page 2, section 2. The authors may want to explicitly state the MJD of the multi-wavelength data that they used in the paper. The optical data points in Figure 2 seem to suggest that the authors are using many epochs of observational data. But Figure 1 seems to show only one epoch of multi-wavelength data. I am confused.

MJDs for all X-ray observations have been noted on line 110 and MJDs for optical polarization measurements have been noted in fig.2's caption. We note sources for the remaining data on line 96 and make clear its non-contemporaneous nature.

5.	Figure 1, in the caption the authors mention grey shaded regions, but I cannot find them. I only see two vertical lines in the X-ray band marking the IXPE range. Is that region supposed to be shaded?

Grey shaded regions around the black SED model line have been made darker and should be clearer in the insets and the main figure panels. Note for some of the blazar states these regions are thin.

6.	Page 2 and 3, section 2.1. Since the model is multi-cell, the authors may want to describe how many cells they used and how they set up the magnetic field morphology. Although the authors cite their previous papers, several things are still unclear. Do they simply draw random numbers for the magnetic field? If so, then the magnetic field morphology is chaotic instead of turbulent. Depending on how they set up the magnetic field, the number of cells is also an important parameter. For instance, in a turbulent setup, the number of cells may reflect how well they resolve the turbulence correlation length, which is an important parameter for the magnetic field morphology.

The number of magnetic field cells for each model are listed in table 2, now brought out of the appendix and into the main text. We revamp the discussion of the model setup, lines 132 -- 176, making clear how magnetic fields are seeded, how the number of magnetic field cells is selected, and the typical resolved correlation length.  

7.	Same place. Do they consider shock and magnetic reconnection scenarios in their magnetic field setup? These two scenarios can potentially lead to very different X-ray polarization degree and energy-dependent polarization in general.

In the model setup discussion, lines 162 -- 176, we mention our mostly acceleration method agnostic setup and move further discussion of acceleration methods to section 4. In section 4, lines 313 -- 350, we discuss the additional effects on polarization we expect from shock and magnetic reconnection acceleration scenarios.

8.	Page 3, line 194. Just curious, is this ixpeobsim tool publicly available now?

It is not yet publicly available, although it will be very soon; the next HEASARC release should contain some of its important functionality.

9.	For the simulation using ixpeobsim, what is the assumption here? Same flux same polarization for the entire duration? Are the model predictions steady-state? I ask because it appears that their previous papers mention the code has light travel time effect, which is usually used in time-dependent models.

Model predictions are steady state, this is now more clearly described in section 2.1 (see point 6 above). The ixpeobssim simulations assume a fixed polarization and flux for the duration of the observation. The polarization and flux are fixed to their expected (average) values based on our model predictions (the black lines in figs 1 and 2). This is now made more clear in the text on lines 238--240. Note that on lines 286--295 we discuss the effects of blazar polarization variability during observation on our predictions.
Light travel time effects can be important in a steady state model too; with such effects, more emission zones are visible far downstream in the jet, as the jet expands and the emitted light overtakes the jet material.

10.	Page 4, line 265. The authors may want to mention that some previous works suggest that TXS 0506+056 is an FSRQ that pretends to be a BL Lac. If that is true, then the polarization degree may be further down in a leptonic model.

Now mentioned on lines 310-312.

11.	Figure 2. It appears that the SSC polarization does not change with energy. But both Bonometto et al. and Zhang & Boettcher show that the SSC polarization rises in higher energy band. What may cause this difference?

SSC polarization does change with energy, just more slowly for the energy ranges displayed than the Zhang & Boettcher single zone model, see point 12 below.

12.	Finally, the polarization predictions for TXS 0506+056 appear different from Zhang et al. 2019, which also considers an SSC model. That paper shows a gradual rise of the polarization degree from less than 5\% in the X-ray band to close to 10\% in the MeV band. Is it because the authors are using different multi-wavelength data? It would be good to add some general comparisons between the two papers since they are the very few papers that provide multi-wavelength polarization predictions for TXS 0506+056.

Lines 208 -- 227 now give a direct comparison between Zhang et al. 2019 and our predictions for a purely leptonic SSC model. In summary, the differences arise from multizone vs. single zone models.

We recommend that living code on github repositories place a "frozen" version on Zenodo (or other 3rd party repositories that issue DOIs) and then cite them in the article. 

We have done so, saving our software on Zenodo and citing it in the text, line 201.

\end{document}

==> referee_response.tex <==
\begin{document}
\textbf{Referee Response}

However, the model is not sufficiently described. It is hard to determine if the model assumptions can broadly reflect the true physical conditions in these blazars. Additionally, there is a previous work on TXS 0506+056 high-energy polarization, which appears to predict slightly different polarization degree. Therefore, I would recommend the authors to expand their description and discussion. It may be better to move the paper to ApJ.
 
1.	Page 1, since both electron synchrotron, proton synchrotron, and pair synchrotron are mentioned in the text, it would be good to explicitly distinguish them to avoid confusion. For instance, in line 57 "the synchrotron" probably means electron synchrotron, in line 58 "synchrotron" probably means electron synchrotron as well, but if the authors refer to the proton synchrotron, depending on the parameters, protons may not cool efficiently in the blazar zone. As long as the acceleration continues, protons can fill up most of the blazar zone easily.

Where appropriate throughout the text, reference to "synchrotron" emission has been disambiguated, making clear where we mean primary electron synchrotron, proton synchrotron, and secondary pair cascade synchrotron.

2.	Page1, line 61, "this means ...". This statement is generally true. However, PIC simulations suggest that the particles and magnetic field distributions are quite chaotic in the turbulent region. In that case, even though there are less cells with high-energy particles, the local PA is very disordered, so that the Stokes parameters can still be canceled easily.

Qualified the statement by noting that this also increases polarization variability, line 62.
As long as downstream of the acceleration region the magnetic fields are equally chaotic, averaging over fewer magnetic field zones always increases the expected (average) polarization. 
We discuss the case where magnetic fields are more or less chaotic close to the acceleration region (than downstream) in more detail in section 4, line 333. Here we mention that immediately downstream of a shock, magnetic fields are more likely to be perpendicular to the shock normal.

3.	Page 2, line 71, "proton-synchrotron". Most leptohadronic models of TXS 0506+056 use photomeson initiated hadronic cascading pair synchrotron to explain the neutrino event and fit SED, including Gao et al. Proton synchrotron is only discussed by very few works, and in those works, proton synchrotron generally dominates the high-energy spectral component. I assume the authors mean the subdominant pair synchrotron.

We have disambiguated "proton synchrotron", line 73; we indeed meant synchrotron from proton initiated cascades. See point 1.

4.	Page 2, section 2. The authors may want to explicitly state the MJD of the multi-wavelength data that they used in the paper. The optical data points in Figure 2 seem to suggest that the authors are using many epochs of observational data. But Figure 1 seems to show only one epoch of multi-wavelength data. I am confused.

MJDs for all X-ray observations have been noted on line 110 and MJDs for optical polarization measurements have been noted in fig.2's caption. We note sources for the remaining data on line 96 and make clear its non-contemporaneous nature.

5.	Figure 1, in the caption the authors mention grey shaded regions, but I cannot find them. I only see two vertical lines in the X-ray band marking the IXPE range. Is that region supposed to be shaded?

Grey shaded regions around the black SED model line have been made darker and should be clearer in the insets and the main figure panels. Note for some of the blazar states these regions are thin.

6.	Page 2 and 3, section 2.1. Since the model is multi-cell, the authors may want to describe how many cells they used and how they set up the magnetic field morphology. Although the authors cite their previous papers, several things are still unclear. Do they simply draw random numbers for the magnetic field? If so, then the magnetic field morphology is chaotic instead of turbulent. Depending on how they set up the magnetic field, the number of cells is also an important parameter. For instance, in a turbulent setup, the number of cells may reflect how well they resolve the turbulence correlation length, which is an important parameter for the magnetic field morphology.

The number of magnetic field cells for each model are listed in table 2, now brought out of the appendix and into the main text. We revamp the discussion of the model setup, lines 132 -- 176, making clear how magnetic fields are seeded, how the number of magnetic field cells is selected, and the typical resolved correlation length.  

7.	Same place. Do they consider shock and magnetic reconnection scenarios in their magnetic field setup? These two scenarios can potentially lead to very different X-ray polarization degree and energy-dependent polarization in general.

In the model setup discussion, lines 162 -- 176, we mention our mostly acceleration method agnostic setup and move further discussion of acceleration methods to section 4. In section 4, lines 313 -- 350, we discuss the additional effects on polarization we expect from shock and magnetic reconnection acceleration scenarios.

8.	Page 3, line 194. Just curious, is this ixpeobsim tool publicly available now?

It is not yet publicly available, although it will be very soon; the next HEASARC release should contain some of its important functionality.

9.	For the simulation using ixpeobsim, what is the assumption here? Same flux same polarization for the entire duration? Are the model predictions steady-state? I ask because it appears that their previous papers mention the code has light travel time effect, which is usually used in time-dependent models.

Model predictions are steady state, this is now more clearly described in section 2.1 (see point 6 above). The ixpeobssim simulations assume a fixed polarization and flux for the duration of the observation. The polarization and flux are fixed to their expected (average) values based on our model predictions (the black lines in figs 1 and 2). This is now made more clear in the text on lines 238--240. Note that on lines 286--295 we discuss the effects of blazar polarization variability during observation on our predictions.
Light travel time effects can be important in a steady state model too; with such effects, more emission zones are visible far downstream in the jet, as the jet expands and the emitted light overtakes the jet material.

10.	Page 4, line 265. The authors may want to mention that some previous works suggest that TXS 0506+056 is an FSRQ that pretends to be a BL Lac. If that is true, then the polarization degree may be further down in a leptonic model.

Now mentioned on lines 310-312.

11.	Figure 2. It appears that the SSC polarization does not change with energy. But both Bonometto et al. and Zhang & Boettcher show that the SSC polarization rises in higher energy band. What may cause this difference?

SSC polarization does change with energy, just more slowly for the energy ranges displayed than the Zhang & Boettcher single zone model, see point 12 below.

12.	Finally, the polarization predictions for TXS 0506+056 appear different from Zhang et al. 2019, which also considers an SSC model. That paper shows a gradual rise of the polarization degree from less than 5\% in the X-ray band to close to 10\% in the MeV band. Is it because the authors are using different multi-wavelength data? It would be good to add some general comparisons between the two papers since they are the very few papers that provide multi-wavelength polarization predictions for TXS 0506+056.

Lines 208 -- 227 now give a direct comparison between Zhang et al. 2019 and our predictions for a purely leptonic SSC model. In summary, the differences arise from multizone vs. single zone models.

We recommend that living code on github repositories place a "frozen" version on Zenodo (or other 3rd party repositories that issue DOIs) and then cite them in the article. 

We have done so, saving our software on Zenodo and citing it in the text, line 201.

\end{document}
